Evolution of a Web-Scale Near Duplicate Image Detection System

Detecting near duplicate images is fundamental to the content ecosystem of photo sharing web applications. However, such a task is challenging when involving a web-scale image corpus containing billions of images. In this paper, we present an efficient system for detecting near duplicate images across 8 billion images. Our system consists of three stages: candidate generation, candidate selection, and clustering. We also demonstrate that this system can be used to greatly improve the quality of recommendations and search results across a number of real-world applications. In addition, we include the evolution of the system over the course of six years, bringing out experiences and lessons on how new systems are designed to accommodate organic content growth as well as the latest technology. Finally, we are releasing a human-labeled dataset of ~53,000 pairs of images introduced in this paper.

==> methods-cg-augmentation.tex <==
\subsubsection{Candidate Augmentation}
The key observation is if query image doesn't match cluster head, it may match some other images in the cluster - even those that are extremely similar to the cluster head. To illustrate, let’s assume we have a cluster "A <-- {B:99,C:99,D:90}" where A is the cluster head, the similarity scores with respect to A are as listed (scale 0-100). Let's say we have query image Q that scores relatively poorly with cluster head - say sim(A,Q) = 10, which is below the current threshold of 65. The key is observation is that sim(B,Q) or sim(C,Q) may be >= 65 even though B and C are extremely close to A. Combination of (A,Q) presents a difficult or adversarial example for the trained classifier, but other images may not be necessarily share that characteristic.


